Theoretical Analysis of Auto Rate-Tuning by Batch Normalization

Batch Normalization (BN) has become a cornerstone of deep learning across diverse architectures, appearing to help optimization as well as generalization. While the idea makes intuitive sense, theoretical analysis of its effectiveness has been lacking. Here theoretical support is provided for one of its conjectured properties, namely, the ability to allow gradient descent to succeed with less tuning of learning rates. It is shown that even if we fix the learning rate of scale-invariant parameters (e.g., weights of each layer with BN) to a constant (say, $0.3$), gradient descent still approaches a stationary point (i.e., a solution where gradient is zero) in the rate of $T^{-1/2}$ in $T$ iterations, asymptotically matching the best bound for gradient descent with well-tuned learning rates. A similar result with convergence rate $T^{-1/4}$ is also shown for stochastic gradient descent.

==> network.tex <==
\section{A specific neural network satisfying the assumptions} \label{sec:network}

In this section, we give a specific example of neural network whose loss function satisfies the assumptions in Section \ref{sec:full} and \ref{sec:stochastic}, and then we apply the convergence results in Section \ref{sec:full} and \ref{sec:stochastic} to show that BatchNorm indeed makes the training less sensitive to the learning rate. This network is a simple feedforward neural networks with a slight variant of BatchNorm. We design the network in a way that only the last layer contains scale-variant parameters, and all other parameters are scale-invariant.

\subsection{Smoothed BatchNorm}

%Recall that the original version of BatchNorm is
In practice, if the original outputs of a neuron over a batch are $\vw^{\top} \vx_1, \dots, \vw^{\top} \vx_B$, then after a BatchNorm layer,
\[
\BN(\vw^{\top} \vx_b) = \gamma \frac{\vw^{\top} \vx_b - \mu}{\sqrt{\sigma^2 + \epsilon}} + \beta,
\]
where $\mu = \E_{b\in[B]}[\vw^{\top} \vx_b]$ and $\sigma^2 = \E_{b\in[B]}[(\vw^{\top} \vx_b - \mu)^2]$ are the mean and variance of the original outputs, $\gamma$ and $\beta$ are two learnable parameters which rescales and offsets the normalized outputs to retain the representation power. To avoid the problem of dividing by zero, \cite{ioffe2015batch} add a small constant $\epsilon > 0$ to the denominator. However, adding a constant $\epsilon$ directly to the denominator breaks the scale-invariant property of $\vw$.

For theoretical analysis, we smooth the classic version of BatchNorm in another way in which it also ensures scale-invariant property of $\vw$. Letting $\vu = \E_{b \in [B]}[\vx_b]$ and $\mS = \Var_{b \in [B]}(\vx_b) = \E[(\vx_b - \vu)(\vx_b - \vu)^\top]$, by simple linear algebra, the classic BatchNorm can also be written as
\[
\BN(\vw^{\top} \vx_b) = \gamma \frac{\vw^{\top} (\vx_b - \vu)}{\sqrt{\|\vw\|^2_{\mS} + \epsilon}} + \beta.
\]
Instead of adding a constant $\epsilon$ directly, we add $\epsilon \|\vw\|^2_2$, which is proportional to $\|\vw\|_2$, to the denominator. Then we can obtain a new variant of BatchNorm, which we call \textit{Smoothed BatchNorm}:
\begin{equation}
\widehat{\BN}(\vw, \vx_b) := \gamma \frac{{\vw}^\top (\vx_b - \vu) }{\left\| \vw \right\|_{\mS + \epsilon \mI}} + \beta.
\end{equation}

\subsection{Network structure}

We introduce a simple feedforward neural network with Smoothed BatchNorm, designed for classification tasks. Let $\Data$ be a data set, consisting of data points in the form of $(\vx, y)$. Here $\vx \in \R^d$ is an input object we want to classify, and $y \in [C]$ is the ground-truth label.

Now we define the network $\Phi$ we intend to study. Let $\vz \sim \Data^B$ be a mini-batch consisting of $B$ data points, $(\vx_1, y_1), \dots, (\vx_B, y_B)$. For each $(\vx_b, y_b)$, let $\xui{0}_b := \vx_b$.
The network consists of $L + 1$ layers, numbered from $0$ to $L$, and $m_0, \dots, m_L$ are the width of each layer ($m_0 = d, m_L = C$).

Given the input $\xui{i-1}_b$, the $i$-th layer first linearly transforms $\xui{i-1}_b$ with weight matrix $\Wui{i} = (\wui{i,1}, \dots, \wui{i,m_i})^\top \in \R^{m_i \times m_{i-1}}$, then it further transforms the output by a smoothed BatchNorm, resulting a vector $\tzui{i}_b \in \R^m$.
\begin{equation}
%\evtzui{i}_{b,k} := \frac{{\wui{i,k}}^\top{\xui{i-1}_b} - \E_{b' \in [B]}\left[{\wui{i,k}}^\top {\xui{i-1}_{b'}}\right]}{\sqrt{\Var_{b' \in [B]}\left({{\wui{i,k}}^\top {\xui{i-1}_{b'}}}\right) + \delta \|\wui{i,k}\|_2^2}}
\evtzui{i}_{b,k} := \widehat{\BN}(\wui{i,k}, \xui{i-1}_b)
%\frac{{\wui{i,k}}^\top{\xui{i-1}_b} - \E_{b' \in [B]}\left[{\wui{i,k}}^\top {\xui{i-1}_{b'}}\right]}{\left\| \wui{i, k} \right\|_{\Sui{i-1} + \epsilon \mI}},
%\sqrt{\Var_{b' \in [B]}\left({{\wui{i,k}}^\top {\xui{i-1}_{b'}}}\right) + \delta \|\wui{i,k}\|_2^2}}
\end{equation}
Let $\gamma^{(i)}_k, \beta^{(i)}_k$ be the corresponding scale and shift parameters in the Smoothed BatchNorm.
%Finally, $\tzui{i}_b$ is processed by a non-linear function.
For $1 \le i < L$, we fix the values of $\gamma^{(i)}_k, \beta^{(i)}_k$ during training (set to $1$ and $0$, or use Gaussian initialization; see Remark \ref{remark:fixed-gamma-beta} for a discussion), and $\tzui{i}_b$ is then processed by a twice continuously differentiable non-linear activation $\sigma$:
\begin{equation}
    \evxui{i}_{b,k} := \sigma(\evtzui{i}_{b,k}).
\end{equation}
For $i = L$, $\gamma^{(L)}_k, \beta^{(L)}_k$ are learnable, and we define $\evxui{L}_{b,k} := \evtzui{i}_{b,k}$ to be the final output of the network.

Let $W = \{ \vw_{i,j} \mid 1 \le i \le L, 1 \le j \le m_i \}$ and $\vg$ consists of all $\gamma^{(L)}_k$ and $\beta^{(L)}_k$. The loss function associated with the mini-batch $\vz$ is a softmax cross-entropy loss with a weight decay $\lambda > 0$ on $\vg$, defined as \footnote{Our results still hold if we do not add the weight decay to $\beta$ (using a slightly complicated argument), but it is necessary in our analysis to add a weight decay to $\gamma$.}
\begin{equation}
    \LossF_{\vz}(W; \vg) := - \frac{1}{B} \sum_{b=1}^{B} \log \frac{\exp(\evxui{L}_{b,y_b})}{\sum_{k = 1}^{C} \exp(\evxui{L}_{b,k})} + \frac{\lambda}{2} \|\vg\|_2^2.
\end{equation}
And we define the expected loss $\Loss(W; \vg) := \E_{\vz \sim \Data^{B}}\left[ \LossF_{\vz}(W; \vg) \right]$ to be the loss values averaged over all the possible mini-batches.

%For $i = L$, we rescales and offsets $\evtzui{i}_{b,k}$ by a learnable scaling factor $\gamma_k$ and a learnable shift parameter $\beta_k$:
%\begin{equation}
%    \evxui{L}_{b,k} := \gamma_k \cdot \evtzui{L}_{b,k} + \beta_k.
%\end{equation}

\begin{remark} \label{remark:fixed-gamma-beta}
Note that during training we fix the scale-variant parameters $\gamma^{(i)}_k$ and $\beta^{(i)}_k$ in all the layers $0 \le i < L$ (but we do not fix them in the last layer). This could eliminate the representation power, but it also has the benefit of preventing from getting stuck in saturated nonlinearities (for activations such as sigmoid). Since the scale and shift parameters in the last layer are still learnable, the network still has the potential to represent functions of any scale.
%Focusing on the smooth setting, we have to fix $\gamma^{(i)}_k$ and $\beta^{(i)}_k$ in internal layers since they are scale-variant.
\end{remark}

\begin{lemma} \label{lam:structure-constants}
There exists constants \footnote{Note that $\Lvv{ij}, \Lvg{i}$ may have an $O(M^L)$ dependence on the maximum width $M = \max\{m_1, \dots, m_L\}$ and the depth $L$.} $\Lvv{ij}, \Lvg{i}, \Lgg, \Gg$ such that
\[
\left\|\frac{\partial}{\partial \vui{i} \partial \vui{j}} \LossF_{\vz}(V; \vg)\right\|_2 \le \Lvv{ij}, \qquad
    \left\|\frac{\partial}{\partial \vui{i} \partial \vg} \LossF_{\vz}(V; \vg)\right\|_2 \le \Lvg{i},
    \qquad
    \left\|\nabla_{\vg}^2 \LossF_{\vz}(V; \vg)\right\|_2 \le \Lgg
\]
and
\[
\E\left[\left\| \nabla_{\vg} \LossF_{\vz}(V; \vg) - \E_{\vz \sim \Data}\left[\nabla_{\vg} \LossF_{\vz}(V; \vg)\right] \right\|^2_2\right] \le \Gg^2
\]
for all $\tilde{\vtheta} = (V; \vg)$ in some set which contains the set of $\tilde{\vtheta}$ associated with the points lying between each pair of $\vtheta_t$ and $\vtheta_{t+1}$ (including the endpoints).
In particular, $\Lgg \le C/2 + \lambda$.
\end{lemma}

We defer the proofs to Appendix \ref{sec:appendix-structure}. Combining with the convergence results in Section \ref{sec:full} and \ref{sec:stochastic}, we can show:
\begin{theorem} \label{thm:structure-main-result}
Let $\Phi$ be the network introduced above. Assume that we initialize the parameters in a way that the initial norm of each weight in $W$ is $O(1)$ and the inital loss value is $O(1)$.
\begin{enumerate}
    \item In full-batch training by gradient descent, we can set the learning rate for $W$ to be arbirary $\etaw > 0$, then $\Phi$ converges to a stationary point in the rate of $O(T^{-1/2})$ as long as $\etagt{t}$ is set to a fixed learning rate $\etag = 4(1 - \cg) / (C + 2\lambda)$ for some constant $\cg \in (0, 1)$;
    \item In mini-batch training by stochastic gradient descent, we can set the learning rate for $W$ to be $\etawt{t} = \etaw (t+1)^{-\alpha}$ with arbitrary $\etaw > 0$ and $0 \le \alpha \le 1/2$, then $\Phi$ converges to a stationary point in the rate of $O(T^{-1/4} \polylog(T))$ as long as $\etagt{t}= \etag (t+1)^{-1/2}$ with $\etag = 4(1 - \cg) / (C + 2\lambda)$ for some constant $\cg \in (0, 1)$.
\end{enumerate}
\end{theorem}

For example, in binary classification tasks, $C = 2$. If $\lambda$ is set to $0.01$, then Theorem \ref{thm:structure-main-result} implies that any $\etag < 1.9$ can work. Thus, for this network, we are able to set the learning rate without considering the data distribution, initialization, etc., and still have the optimal asymptotic convergence rate.

==> noisy.tex <==
\section{Training by Noisy Gradient Descent} \label{sec:noisy}

In this section, we rigorously analyze the effect related to the scale-invariant properties in training neural network by gradient descent with manually injecting noise.

\subsection{Settings}

We follow the setting from Section \ref{sec:full}.

We focus on the case that $W = \{\vw\}$ for $\vw \in \R^d$ and there is no $\vg$.

We use $\Lvv{}$ to be the upper bound of $\left\| \nabla^2 \mathcal{L}(V) \right\|_2$, where $V = \{\vv\}$ and $\vv = \vw / \|\vw\|_2$.

\paragraph{Training with Injecting Noise.} The update rule is %In order to illustrate the optimization benefits of scale-invariant properties, we consider the process of training this neural network by gradient descent with separate learning rates for $W$ and $\vg$. More specifically, 
\begin{align}
    \vw_{t+1} &\gets \wui{i}_t - \etaw \left(\nabla_{\wui{i}_t} \mathcal{L}(\vw_t) + \xi_t \right),
\end{align}
where $\xi_t$ is sampled uniformly at random from the sphere of radius $\frac{\sigma}{\|\vw_t\|_2}$ in the plane perpenticular to $\vw_t$, namely, $\{ \vu \in \R^d \mid \vu \cdot \vw_t = 0, \|\vu\|_2 = \frac{\sigma}{\|\vw_t\|_2} \}$. For ease of notation, define $\Delta \vw_t = - \etaw \nabla_{\vw_t} \mathcal{L}(\vw_t) + \frac{\sigma}{\|\vw_t\|_2}\xi_t$.

\kaifeng{We are thinking about how to generalize it}

\subsection{Main Theorem}

\begin{theorem}
Not sure
\end{theorem}

\subsection{Proof Sketch}

Step 1. $\|w_t\| \sim T^{1/4}$ w.h.p.

Step 2. Use a lemma from Rong's paper

Step 3. Analyze a stochastic process: time += 1 and func -= $1/T$ or time += $1/\sqrt{T}$ and func -= $1/\sqrt{T}$.

==> prelim.tex <==
\section{Backgrounds} \label{sec:back}

Let $C$ be a convex set. For a function $f: C \to \R$, we say that $f$ is $\lipG$-Lipschitz if for all $\vx, \vy \in C$,
\begin{equation}
    \lvert f(\vx) - f(\vy) \rvert \le \lipG \|\vx - \vy\|_2.
\end{equation}
We say that $f$ is $\smtL$-smooth if for all $\vx, \vy \in C$,
\begin{equation}
    \left\| \nabla f(\vx) - \nabla f(\vy) \right\|_2 \le \smtL \|\vx - \vy\|_2.
\end{equation}

For a matrix $A$, we use $\|\mA\|_2$ to denote the operator $\ell_2$-norm, $\lammin(\mA)$ to denote the minimum eigenvalue, and $\lammax(\mA)$ to denote the maximum eigenvalue. The condition number of a matrix $\mA$ is defined as $\lammax(\mA) / \lammin(\mA)$.

\begin{comment}
\subsection{Convergence of Gradient Descent}

Now we recall the classical result for showing convergence of gradient descent (see, e.g., \cite{jain2017non} for more details). For $\smtL$-smooth function $\mathcal{L}(\theta)$, when optimizing by gradient descent $\theta_{t+1} = \theta_t - \eta \nabla \mathcal{L}(\theta_t)$, it is a conventional result that by Taylor expansion
\begin{align*}
\mathcal{L}(\theta_{t+1}) &\le \mathcal{L}(\theta_{t}) - \eta \nabla \mathcal{L}(\theta_{t})^\top \nabla \mathcal{L}(\theta_{t}) + \frac{\smtL}{2} \eta^2 \left\| \nabla \mathcal{L}(\theta_{t}) \right\|_2^2 \\
&\le \mathcal{L}(\theta_{t}) - \eta \left(\eta - \frac{\smtL}{2}\right) \left\| \nabla \mathcal{L}(\theta_{t}) \right\|_2^2.
\end{align*}
Thus, for $\eta < \frac{2}{\smtL}$, gradient descent successively decreases the loss and converges to a stationary point. One can also easily construct examples in which gradient descent diverges if $\eta > \frac{2}{\smtL}$.
\end{comment}

